Solving polynomial systems via homotopy continuation and monodromy

We study methods for finding the solution set of a generic system in a family of polynomial systems with parametric coefficients. We present a framework for describing monodromy based solvers in terms of decorated graphs. Under the theoretical assumption that monodromy actions are generated uniformly, we show that the expected number of homotopy paths tracked by an algorithm following this framework is linear in the number of solutions. We demonstrate that our software implementation is competitive with the existing state-of-the-art methods implemented in other software packages.

==> generalizations.tex <==
The goal of this article and our implementation is to demonstrate the power of the main algorithm and analyze it in the simplest terms possible. 
This section collects possible modifications, extensions, and ideas for the future that we purposefully excluded from the main scope of this paper.  
One topic for future development is the stopping criterion using the trace test as discussed in Remark~\ref{rem:trace-test}. 
%We already brought up one topic for future development---the stopping criterion using the trace test--- 
Some of the modifications of our algorithm are relatively straightforward (e.g., \S\ref{sec:Galois}); however, their careful implementation is not. Accompanied with careful analysis, this should be carried out elsewhere. 

\subsection{Numerical failures}\label{sec:failures}
One advantage of our approach is that it can tolerate numerical failures of the underlying homotopy tracker. Such failures are bound to happen as the size of problems increases and the probability of a path going too close to the discriminant 
%(i.e., encountering large condition numbers) 
gets higher. The canonical remedy is increasing computational precision either uniformly or adaptively. However, this tends to result in much higher computational costs.

When the tracking of a homotopy path in Algorithm~\ref{alg:sgs} fails, one could simply record that the starting point of that path corresponds to a failure. The algorithm then avoids retracking this path, while its target solution still has high chances to be reached by some path along a different edge.
In fact, we already implemented this simple failure resistant mechanism and it successfully tolerates a few failures that arise in some runs for large test examples in~\S\ref{sec:timings}.
What has yet to be done is the statistical analysis in the presense of failures, under some suitable assumptions, and modifications of heuristic strategies, e.g., edge potential functions may penalize failures. 

\subsection{Nonlinear families}\label{sec:nonlinear}
Let us reiterate that we choose to restrict ourselves to families of polynomial systems $F_p$ that are affine linear in parameters for the sake of simplicity of exposition. Also, as pointed out in Remark~\ref{rem:parameter-segment-homotopy}, if a family is nonlinear in parameters, then the ability to replace systems with their scalar multiples is lost, together with an inexpensive way to produce new homotopies between two nodes in our graph.
If a family is nonlinear, the ingredients in the algorithm that should change are the following.
\begin{itemize}
\item There could be only one edge between two nodes, since $\gamma_1$ and $\gamma_2$ have to be equal to $1$ (see the discussion above).
\item The initial seed, a parameter-solution pair $(p_0,x_0)$, can not be produced in the same simple manner. One can still pick a solution $x_0$ at random, but the system $F_{p}(x_0)=0$ will not be linear in parameters $p$. 
One has to find generic points on \emph{all} solution components of this system and use them as seeds in order to eventually capture all solutions of a generic system. % The components would have to include, in particular, the embedded components of the scheme defined by the polynomials $F_{p}(x_0)$.  
\item Since the dominant component of the solution variety (cf.~Remark~\ref{rem:dominant-component}) is not necessarily irreducible anymore, the relevance of our statistical analysis based on modelling the monodromy group as a symmetric group is further reduced.
\end{itemize} 

\subsection{Arbitrary parameter varieties} 
We assumed that the parameter space is a complex affine space. In fact, one can drop this assumption and consider the family given by a \defn{rational} map $\phi$ from an irreducible variety of parameters $P$ to the space of polynomial systems. 
Our algorithm would still work as long as given two points in $P$ one has a way to construct a parametrization of a curve containing these points. 

Note that even in the case of the whole affine space, one doesn't need to stick linear segment homotopies. Should some family of explicitly constructible curves present a faster way to generate the monodromy group, the algorithm could associate edges in the graph to segments of those curves.

\subsection{Monodromy/Galois group computation}\label{sec:Galois}
The classical article in enumerative geometry \cite{Harris:Galois-groups} points out that a Galois group can be defined as the monodromy group of a covering map.
Various interesting theoretical questions related to Galois groups of incidence varieties (called solution varieties here) can be attacked by a monodromy group computation, see~\cite{Leykin-Sottile:HoG,hauenstein2016numerical}. 

Suppose our algorithm is set to stop when the correspondences are saturated. That is, when for every edge $e = v_i \xleftrightarrow{} v_j$ there is a bijection of full solution sets for the nodes $v_i$ and $v_j$. 
Assuming there are no failures discussed in~\S\ref{sec:failures},  one can construct a subgroup of the monodromy group induced by the fundamental group of the graph using complete correspondences between the points of the fibers along every edge by simply collecting the permutations corresponding to the simple cycles. 
This modification gives a heuristic algorithm to compute Galois groups.  In certain scenarios (e.g.,~\cite{Leykin-Sottile:HoG}) the Galois group is the largest one possible, the symmetric group, which provides an obvious verification procedure.
In general, we know no good way (apart from computing the discriminant locus and, therefore, the fundamental group; which is an option only for toy problems) to design a stopping criterion that guarantees that the subgroup is actually the entire Galois group.

\subsection{Parallelization}
Homotopy continuation is \defn{embarrassingly parallel}, since homotopy continuation paths can be tracked independently. A naive parallelization strategy for our approach is to pick an edge and direction according to~\S\ref{sec:edgeselection}, one point in the source vertex that has no correspondence along that edge, and task an idling processor with tracking the path emanating from that point. 
This would likely suffice to achieve linear speedups asymptotically as the number of processors is fixed while the number of solutions grows.  

However, firstly, in various stages of computation the number of eligible paths may drop below the number of available idling processors. This phenomena may happen not only close to the beginning---it starts with one point---and the end of computation, but also in the intermediate stages. 
Secondly, the tasks as described are not completely independent, since the outcome of a task affects the procedure of selection of the next task. The efficiency of a naive parallelization may also decrease due to the fact that there is a non-zero probability for two paths with the same vertex as a target to produce the same point.

An asynchronous approach of~\cite{Ley-Ver-new-monodromy-05} demonstrates the nontriviality of the problem of parallelization in a similar setting. 
One should look carefully at how to modify potentials in~\S\ref{sec:edgeselection} in case several tracking tasks that are ``in progress''. This may be even less trivial if numerical failures discussed in~\S\ref{sec:failures} are taken into account.   

\subsection{Hybrid approaches}
Our algorithm has yet another flexible feature. Suppose one has a method to generate partial solution sets for a given value of parameters. Then that method can be combined with our method  in several ways.
One way is through preprocessing by initializing Algorithm~\ref{alg:sgs} with partial solution sets $Q'_i$ computed with that method. An interesting combination to explore would be using polyhedral homotopies to populate just one set of known points, e.g. $Q'_1$. One could discard paths that are poorly conditioned, thus producing a solution set that is potentially incomplete but is computed very fast.   
Another way would be to combine any solver that produces random points in the fibers \emph{in parallel} with the procedure that discovers new points in Algorithm~\ref{alg:sgs}. This has a potential to produce a faster and more robust blackbox solver by employing the best qualities of all methods involved.

% LocalWords:  parallelization

